Parsing Linear Context-Free Rewriting Systems with Fast Matrix Multiplication

We describe a matrix multiplication recognition algorithm for a subset of binary linear context-free rewriting systems (LCFRS) with running time $O(n^{\omega d})$ where $M(m) = O(m^{\omega})$ is the running time for $m \times m$ matrix multiplication and $d$ is the "contact rank" of the LCFRS -- the maximal number of combination and non-combination points that appear in the grammar rules. We also show that this algorithm can be used as a subroutine to get a recognition algorithm for general binary LCFRS with running time $O(n^{\omega d + 1})$. The currently best known $\omega$ is smaller than $2.38$. Our result provides another proof for the best known result for parsing mildly context sensitive formalisms such as combinatory categorial grammars, head grammars, linear indexed grammars, and tree adjoining grammars, which can be parsed in time $O(n^{4.76})$. It also shows that inversion transduction grammars can be parsed in time $O(n^{5.76})$. In addition, binary LCFRS subsumes many other formalisms and types of grammars, for some of which we also improve the asymptotic complexity of parsing.

==> Makefile <==
.PHONY: dvi ps pdf all space clean veryclean distclean

SHELL = /bin/sh
MAKE  = gmake

# latex --interaction {batchmode, nonstopmode, scrollmode, errorstopmode}
#TEX = latex --interaction batchmod
TEX = latex  -file-line-error-style
PDFTEX = pdflatex  -file-line-error-style

######################################################################
# source files

texfiles = $(wildcard *.tex)
bibfiles = $(wildcard *.bib)

tblfiles = $(wildcard tbl/*.tex)

styfiles  = $(wildcard *.sty)

figfiles  = $(wildcard img/*.tex)
figfiles += $(wildcard fig/*.plt)
figfiles += $(wildcard fig/*.pdf)
figfiles += $(wildcard fig/*.ps)
figfiles += $(wildcard fig/*.epsi)
figfiles += $(wildcard fig/*.c)

tmp_files = $(wildcard *.log)
tmp_files += $(wildcard *.aux)
tmp_files += $(wildcard *.blg)
tmp_files += $(wildcard *.bbl)
tmp_files += $(wildcard *.toc)
tmp_files += $(wildcard *.dvi)
#tmp_files += (texput.log)

######################################################################
# output files

target = lcfrs2

######################################################################
# make targets

all: pdf

dvi: ${target}.dvi

ps: ${target}.ps

pdf: ${target}.pdf

space:
	@if [ -d fig ]; then cd fig; ${MAKE} $@; fi
	@-/bin/rm -f ${tmp_files} *~ ${target}.pdf ${target}.ps

clean veryclean distclean:
	#	if [ -d fig ]; then cd fig; ${MAKE} $@; fi
	/bin/rm -f ${tmp_files} *~ ${target}.pdf ${target}.ps ${target}.dvi

######################################################################
# rules

%.dvi : %.tex ${figfiles}
	@${TEX} $<
	@if grep -q bibdata ${*F}.aux ; then \
		bibtex ${*F};	\
		${TEX} $<;	\
		bibtex ${*F};	\
	fi
	@${TEX} $<
#	@-/bin/rm -f ${tmp_files}

%.ps : %.dvi
	dvips -P pdf -G0 -q -o $@ $<

%.pdf : %.ps ${figfiles}
	ps2pdf $< $@

#%.pdf : %.tex #${texfiles} ${bibfiles} ${styfiles} ${figfiles} ${tblfiles}
#	@if [ -d fig ]; then cd fig; ${MAKE} all; fi
#	@${PDFTEX} $<
#	@if grep -q bibdata ${*F}.aux ; then \
#		bibtex ${*F};	\
#		${PDFTEX} $<;	\
#		bibtex ${*F};	\
#	fi
#	${PDFTEX} $< $@
#	@-/bin/rm -f ${tmp_files}


#%.bib:	%.aux
#	BSTINPUTS=/u/gildea/src/bibtools-2000/bibtools /u/gildea/src/bibtools-2000/bibtools/aux2bib $<
#	mv references.bib $@


slides.ps : slides.dvi
	dvips -t landscape -P pdf -G0 -q -o $@ $<


######################################################################
# dependences

${target}.dvi: ${texfiles} ${bibfiles} ${styfiles} ${figfiles} ${tblfiles} Makefile

